Concurrent Fixed-Size Allocation and Free in Constant Time

Our goal is to efficiently solve the dynamic memory allocation problem in a concurrent setting where processes run asynchronously. On $p$ processes, we can support allocation and free for fixed-sized blocks with $O(1)$ worst-case time per operation, $\Theta(p^2)$ additive space overhead, and using only single-word read, write, and CAS. While many algorithms rely on having constant-time fixed-size allocate and free, we present the first implementation of these two operations that is constant time with reasonable space overhead.

==> applications.tex <==

\section{Applications to Wait-free Stack}
\label{sec:app}

\Hao{We could have used Hazard Pointers \cite{michael2004hazard} in this stack to avoid..., but it would have increased on time complexity to expected constant time. Since memory allocation is an basic building block for many algorithms, this would make their time bounds \emph{expected} rather than \emph{worst-case}, so we decided against using Hazard Pointers. We believe that allowing the memory allocator to access memory that it has allocated is reasonable.}

We believe this is the first runtime bound for a concurrent stack that accounts for both memory management and memory allocation.

% \subsection{LL/SC from CAS}

% \Hao{Talk about how Maged Michael's ABA prevention using Hazard Pointers requires memory allocation. In general, any algorithm that uses indirection requires memory allocation to allocate the indirect object.}

==> extensions.tex <==

\subsection{Extensions}
\label{sec:extensions}



==> malloc-alg.tex <==

\Hao{I want to argue that local\_batches is not accessed while a delayed operation is happening on it.}

\begin{figure}
\small
\begin{verbatim}
using batch = stack<block>;
shared_stack<batch> shared_pool;
thread_local stack<batch> local_batches; 
thread_local stack<block> alloc_batch; // alloc from here
thread_local stack<block> free_batch; // free to here

block* allocate() {
  if (alloc_batch.empty()) {
    alloc_batch = local_batches.pop();
    if (local_batches.empty()) 
      delayed local_batches.push(shared_pool.pop());
  }
  run_delayed_step();
  return alloc_batch.pop();
}

void free(block* b) {
  if (current_batch.full()) {
    if (num_batches == 2) 
      delayed shared_pool.push(current_batch);
    else {
      num_batches++;
      local_batches.push(current_batch);
    }
    current_batch = empty;
  }
  run_delayed_step();
  current_batch.push(b);
}
\end{verbatim}
\caption{Allocation anf Free}
\label{fig:allocfree}
\end{figure}

==> stack-alg.tex <==

  \begin{figure}[!t!h]
  \begin{lstlisting}[linewidth=\columnwidth, xleftmargin=5.0ex, numbers=left]
struct Block {
  Block* nextBlock;
  Batch* nextBatch; };

struct Stack<Block> {
  Block* head;
  Block* top() { return head; }
  void push(Block* b) {
    b->nextBlock = head;
    head = b; }
  Block* pop() {
    Block* ret = head;
    head = head->nextBlock;
    return ret; } };

using Batch = Block;

struct Stack<Batch> {
  Batch* head;
  Batch* top() { return head; }
  void push(Batch* b) {
    b->nextBatch = head;
    head = b; }
  Batch* pop() {
    Batch* ret = head;
    head = head->nextBatch;
    return ret; } };
  \end{lstlisting}
  \caption{Universal Construction}
  \end{figure}

==> todo.tex <==

\section{Questions for Guy}
\begin{itemize}
  \item Do brief announcements need abstracts?
\end{itemize}

\section{Outline}

\begin{itemize}
  \item The high level idea is that each process has a private pool of memory blocks that it allocates from and frees to.
  \item Once this pool becomes too big the process pushes a batch of nodes to a shared pool. Similarly when the pool becomes too small.
  \item We begin by describing how this shared pool is implemented and then describe how the private pools are maintained.
  \item Shared pool:
  \begin{itemize}
    \item We begin with a sequential stack algorithm which we make concurrent using Youla's universal construction
    \item There are two issues with this algorithm, 1) is the large LL/SC object and 2) is that it doesn't discuss garbage collection.
    \item We modifying the algorithm to handle garbage collection efficiently, and this modification requires relaxing the semantics of the data structure from shared stack to shared pool.
  \end{itemize}
  \item Pseudo-code:
  \begin{itemize}
    \item Instead of OOP, maybe we should have methods called append_block and append_batch, which takes a block pointer as argument
  \end{itemize}
\end{itemize}
